Noncommutative projective curves and quantum loop algebras

We generalize a theorem of Kapranov by showing that the Hall algebra of the category of coherent sheaves on a weighted projective line (over a finite field) provides a realization of the (quantized) enveloping algebra of a certain nilpotent subalgebra of the affinization of the correponding Kac-Moody algebra. In particular this yieds a geometric realization of the quantized enveloping algebra of 2-toroidal (or elliptic) algebras of types D_4, E_6, E_7 or E_8 in terms of weighted projective lines of genus one.

==> StarDynkin <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 4275 5550 4875 5925
4 0 0 50 0 0 16 0.0000 4 225 555 4275 5775 p   -1\001
4 0 0 50 0 0 12 0.0000 4 135 285 4350 5925 n-1\001
-6
6 6075 5550 6600 5925
4 0 0 50 0 0 16 0.0000 4 225 495 6075 5775 p  -1\001
4 0 0 50 0 0 12 0.0000 4 135 90 6225 5925 2\001
-6
6 6975 3975 7500 4350
4 0 0 50 0 0 16 0.0000 4 225 495 6975 4200 p  -1\001
4 0 0 50 0 0 12 0.0000 4 135 90 7125 4350 1\001
-6
6 3300 3975 3900 4350
4 0 0 50 0 0 16 0.0000 4 225 555 3300 4200 p   -1\001
4 0 0 50 0 0 12 0.0000 4 90 90 3450 4350 n\001
-6
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 5400 4500 106 106 5400 4500 5475 4575
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 3150 5850 106 106 3150 5850 3225 5925
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 3150 3150 106 106 3150 3150 3225 3225
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 7650 5850 106 106 7650 5850 7725 5925
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 7650 3150 106 106 7650 3150 7725 3225
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 4650 4050 106 106 4650 4050 4725 4125
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 4650 4950 106 106 4650 4950 4725 5025
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 6150 4950 106 106 6150 4950 6225 5025
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 6150 4050 106 106 6150 4050 6225 4125
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 6900 3600 106 106 6900 3600 6975 3675
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 6900 5400 106 106 6900 5400 6975 5475
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 3900 5400 106 106 3900 5400 3975 5475
1 3 0 1 0 7 50 0 -1 4.000 1 0.0000 3900 3600 106 106 3900 3600 3975 3675
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 4500 6150 4050
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6900 3600 7650 3150
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 4500 6150 4950
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6900 5400 7650 5850
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4650 4050 5400 4500
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 3150 3900 3600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4650 4950 5400 4500
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 5850 3900 5400
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3900 5400 4650 4950
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3900 3600 4650 4050
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6900 3600 6150 4050
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6150 4950 6900 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 4
	 6000 4350 6150 4500 7800 3525 7725 3375
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 4
	 3450 5850 3600 6000 5250 5025 5175 4875
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 4
	 4800 4350 4650 4500 3000 3525 3075 3375
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 4
	 7350 5850 7200 6000 5550 5025 5625 4875
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4950 5700 5850 5700
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4950 5850 5850 5850
4 0 0 50 0 0 16 0.0000 4 165 120 5325 4350 0\001

